System-level, Input-output and New Parameterizations of Stabilizing Controllers, and Their Numerical Computation

It is known that the set of internally stabilizing controller $\mathcal{C}_{\text{stab}}$ is non-convex, but it admits convex characterizations using certain closed-loop maps: a classical result is the Youla parameterization, and two recent notions are the system-level parameterization (SLP) and the input-output parameterization (IOP). In this paper, we address the existence of new convex parameterizations and discuss potential tradeoffs of each parametrization in different scenarios. Our main contributions are: 1) We reveal that only four groups of stable closed-loop transfer matrices are equivalent to internal stability: one of them is used in the SLP, another one is used in the IOP, and the other two are new, leading to two new convex parameterizations of $\mathcal{C}_{\text{stab}}$. 2) We investigate the properties of these parameterizations after imposing the finite impulse response (FIR) approximation, revealing that the IOP has the best ability of approximating $\mathcal{C}_{\text{stab}}$ given FIR constraints. 3) These four parameterizations require no \emph{a priori} doubly-coprime factorization of the plant, but impose a set of equality constraints. However, these equality constraints will never be satisfied exactly in floating-point arithmetic computation and/or implementation. We prove that the IOP is numerically robust for open-loop stable plants, in the sense that small mismatches in the equality constraints do not compromise the closed-loop stability; but a direct IOP implementation will fail to stabilize open-loop unstable systems in practice. The SLP is known to enjoy numerical robustness in the state feedback case; here, we show that numerical robustness of the four-block SLP controller requires case-by-case analysis even the plant is open-loop stable.

==> LTIsetup.tex <==
\setlength{\unitlength}{0.008in}
\begin{picture}(243,115)(140,410)
\thicklines
\put(187,440){\vector(1, 0){ 43}}
\put(180,510){\vector( 0, -1){ 65}}
\put(128,440){\vector( 1, 0){ 48}}
\put(140,445){\makebox(0,0)[lb]{$\delta_{\mathbf{y}}$}}
\put(181,440){\circle{10}}
\put(180,510){\line( 1, 0){ 48.5}}

\put(340,510){\circle{10}}
\put(335,510){\vector( -1, 0){ 45}}
\put(340,439.5){\vector( 0,1){ 65.5}}
\put(290,440){\line(1, 0){ 50}}
\put(393,510){\vector(-1, 0){ 48}}
\put(365,515){\makebox(0,0)[lb]{$\delta_{\mathbf{u}}$}}


\put(230,420){\framebox(60,40){}}
\put(230,490){\framebox(60,40){}}
\put(200,445){\makebox(0,0)[lb]{$\mathbf{y}$}}
\put(315,515){\makebox(0,0)[lb]{$\mathbf{u}$}}
\put(252,435){\makebox(0,0)[lb]{$\mathbf{K}$}}
\put(248,505){\makebox(0,0)[lb]{$\mathbf{P}_{22}$}}
\put(185,450){\makebox(0,0)[lb]{\footnotesize +}}
\put(167,445){\makebox(0,0)[lb]{\footnotesize +}}

\put(350,515){\makebox(0,0)[lb]{\footnotesize +}}
\put(345,498){\makebox(0,0)[lb]{\footnotesize +}}

\end{picture}

